Towards Agentic Proof Harness Engineering

Formal verification of real-world projects requires substantial manual effort, from specifying correctness properties to constructing the infrastructure needed to check them. We envision verification agents that assist developers throughout this process. Among the many tasks involved, one stands out as both foundational and amenable to automation: proof-harness engineering. A proof harness defines an isolated verification environment for a program unit, such as a function or module, by providing symbolic inputs, initialization code, and models of its dependencies. Today, proof-harness engineering remains largely a manual task performed by verification engineers. To explore the potential of coding agents for this task, we propose an agentic proof-harness engineer that automatically constructs verifier-ready harnesses from a software project and a designated verification target. We combine the agent with formal soundness and precision guards to validate generated abstractions and guide their refinement. We evaluate the feasibility of our approach in an exploratory case study on curl and libuv, using three historical assertion violations already embedded in the source code as verification properties. Our results show that the agent successfully constructs proof harnesses that enable CBMC to detect all three violations. We further demonstrate the potential for reusing these harnesses with other verification tools.

==> sections/2_setup.tex <==
\section{Experimental Setup}

\subsection{Agent Rules}
The agent cannot violate the following rules:

\begin{enumerate}
    \item \textbf{Isolated execution.} The agent has access to the  shell, but all commands run inside an isolated docker container, never on the host machine.
     \item \textbf{Clean start.} Each run starts with only the project's source files. Irrelevant things such as results of earlier runs are moved out of reach from the agent.
     \item \textbf{Check before use.} A mock rule can only be added to the harness after it has passed all the checks (Ref \ref{subsec:checks}).
     \item \textbf{Verdicts come from verifier.} The agent may only finish with a verdict that a verifier has actually reported, other verdicts are rejected.
     \item \textbf{Flag empty results.} If a clean result holds only because the mock rules exclude every possible execution, it is reported as \textsc{Vacuous}.
     \item \textbf{Limits.} At most 100 steps per run.
     \item \textbf{Logging.} Every command, its output, and every proposed rule is logged for reference.
     \item \textbf{Access.} Only files in the \texttt{verification/} folder may be created or changed. The source code, headers, build files, or assertions cannot be modified. This is also checked at the code level to ensure the agent obeys this rule.
     \item \textbf{Rules must be general:} a C condition over the return value and the function's parameters, without numbers copied from a counterexample. However, named limits (e.g.\ \texttt{SHRT\_MIN}) and macros(e.g.\ \texttt{RANGE}) are allowed.
     \item \textbf{Integrity.} The agent runs one command per step and the agent must never invent a command's output.
\end{enumerate}
In addition, the prompt and the tool messages guide the model on how to write mock the rules. This affects how quickly the agent can reaches a verdict by avoiding false positives.

\subsection{Verification outcomes}
The following verification outcomes are possible/allowed:
\begin{description}
  \item[\textsc{Violation}] The verifier found inputs that violates an assertion in the harness. This may be a real bug or a false alarm.
  \item[\textsc{Verified\_Clean}] The verifier found no violations in the assertion(s).
  \item[\textsc{Vacuous}] The verifier found no violation, but only because the mock rules leave no possible execution. The result proves nothing.
  \item[\textsc{Verifier\_Error}] The verifier could not run, e.g.\ because the harness does not compile.
\end{description}

\subsection{Replay outcomes} 
The following outcomes are possible when a counterexample is executed on the real program to ensure the verification verdict is not a false alarm.
\begin{description}
  \item[\textsc{Reproduced}] i.e. a \emph{real bug}. The inputs from the counterexample make the real program fail at the same assertion.
  \item[\textsc{Not\_Reproduced}] i.e. a \emph{false alarm}. The real program runs without failure on those inputs.
  \item[\textsc{Guarded}] i.e. \emph{inconclusive}. The real program exits early on those inputs and never reaches the assertion.
\end{description}

\subsection{Rule-checks and outcomes}
\label{subsec:checks}
The following are the outcomes after checking each mock function.
\begin{description}
  \item[\textsc{Not\_Refuted}] The verifier found no input for which the real function violates the proposed rule. The rule may be used.
  \item[\textsc{Refuted}] The verifier found an input for which the real function violates the proposed rule. The rule is too strong and must be weakened.
  \item[\textsc{Error}] The rule could not be checked, e.g.\ because it is not valid (syntax error).
\end{description}
